Learning Hierarchical Discrete Linguistic Units from Visually-Grounded Speech

In this paper, we present a method for learning discrete linguistic units by incorporating vector quantization layers into neural models of visually grounded speech. We show that our method is capable of capturing both word-level and sub-word units, depending on how it is configured. What differentiates this paper from prior work on speech unit learning is the choice of training objective. Rather than using a reconstruction-based loss, we use a discriminative, multimodal grounding objective which forces the learned units to be useful for semantic image retrieval. We evaluate the sub-word units on the ZeroSpeech 2019 challenge, achieving a 27.3\% reduction in ABX error rate over the top-performing submission, while keeping the bitrate approximately the same. We also present experiments demonstrating the noise robustness of these units. Finally, we show that a model with multiple quantizers can simultaneously learn phone-like detectors at a lower layer and word-like detectors at a higher layer. We show that these detectors are highly accurate, discovering 279 words with an F1 score of greater than 0.5.

==> math_notation.tex <==
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}

==> noisy_places_ABX_table_full.tex <==
\begin{table}[h]
    \caption{Comparison of R@10, ABX scores, and bit-rates between models trained on the noisy PlacesAudio dataset.}
    \label{tab:noisy_places_r10_abx_full}
    \begin{center}
    \begin{tabular}{cccc|cccccc}
        \toprule
        \multirow{2}{*}{ID} & \multirow{2}{*}{Init ID} & 
        \multirow{2}{*}{Quant} & \multirow{2}{*}{Feat} & 
        \multirow{2}{*}{R@10} & \multicolumn{3}{c}{Frame-Based} & \multicolumn{2}{c}{Segment-Based} \\
         & & & & & ABX & Bitrate & RLE Bitrate & ABX & Bitrate \\
        \cmidrule(lr){6-8}\cmidrule(lr){9-10}
        \midrule
        \multirow{4}{*}{0} & \multirow{4}{*}{-} & \multirow{4}{*}{N/A} &
              1 & \multirow{4}{*}{.660} & 19.82
              & \multirow{4}{*}{N/A} & \multirow{4}{*}{N/A} 
              & \multirow{4}{*}{N/A} & \multirow{4}{*}{N/A} \\
        & & & 2 & & 12.32 & \\
        & & & 3 & & 11.85 & \\
        & & & 4 & & 15.21 & \\
        \midrule
        2   & - & 2 & 2 & .653 & 13.42 & 424.82 & 364.17 & 13.64 & 337.56 \\
        0-2 & 0 & 2 & 2 & .683 & \textbf{12.64} & 411.98 & 342.53 & 13.23 & 316.28 \\
        \midrule
        3   & - & 3 & 3 & .489 & 34.56 & 218.94 & 184.98 & 35.22 & 167.87 \\
        0-3 & 0 & 3 & 3 & .718 & \textbf{15.35} & 205.53 & 170.86 & 16.50 & 156.63 \\
        \midrule
        \multirow{2}{*}{2,3} & \multirow{2}{*}{-} & \multirow{2}{*}{2,3} 
            & 2 & \multirow{2}{*}{.430} & 25.24 & 422.51 & 281.81 & 25.79 & 239.70 \\
        & & & 3 &                       & 29.72 & 216.72 & 169.68 & 30.08 & 152.37 \\
        \multirow{2}{*}{0-2,3} & \multirow{2}{*}{0} & \multirow{2}{*}{2,3} 
            & 2 & \multirow{2}{*}{.697} & 23.67 & 407.53 & 341.08 & 22.92 & 311.31 \\
        & & & 3 &                       & 21.89 & 184.56 & 160.34 & 22.00 & 147.85 \\
        \multirow{2}{*}{2-2,3} & \multirow{2}{*}{2} & \multirow{2}{*}{2,3} 
            & 2 & \multirow{2}{*}{.654} & \textbf{13.42} & 418.78 & 365.89 & 13.82 & 329.29 \\
        & & & 3 &                       & \textbf{14.39} & 199.24 & 179.19 & 14.71 & 169.58 \\
        \multirow{2}{*}{3-2,3} & \multirow{2}{*}{3} & \multirow{2}{*}{2,3} 
            & 2 & \multirow{2}{*}{.543} & 16.52 & 378.23 & 223.28 & 17.28 & 181.59 \\
        & & & 3 &                       & 26.21 & 217.28 & 187.31 & 26.74 & 173.05 \\
        \bottomrule
    \end{tabular}
    \end{center}
\end{table}

==> noisy_places_ABX_table_short.tex <==
\begin{table}[h]
    \small
    \caption{Comparison of R@10, ABX scores, and bit-rates between models trained on the noisy PlacesAudio dataset. \todo{Move this to appendix? Seems like we can combine the relevant results from this table with Table \ref{tab:noisy_abx}}}
    \label{tab:noisy_places_r10_abx_short}
    \begin{center}
    \begin{tabular}{cccc|cccccc}
        \toprule
        \multirow{2}{*}{ID} & \multirow{2}{*}{Init ID} & 
        \multirow{2}{*}{Quant} & \multirow{2}{*}{Feat} & 
        \multirow{2}{*}{R@10} & \multicolumn{3}{c}{Frame-Based} & \multicolumn{2}{c}{Segment-Based} \\
         & & & & & ABX & Bitrate & RLE Bitrate & ABX & Bitrate \\
        \cmidrule(lr){6-8}\cmidrule(lr){9-10}
        \midrule
        2(n)   & - & 2 & 2 & .653 & 13.42 & 424.82 & 364.17 & 13.64 & 337.56 \\
        0-2(n) & 0(n) & 2 & 2 & .683 & \textbf{12.64} & 411.98 & 342.53 & 13.23 & 316.28 \\
        \midrule
        3(n)   & - & 3 & 3 & .489 & 34.56 & 218.94 & 184.98 & 35.22 & 167.87 \\
        0-3(n) & 0(n) & 3 & 3 & .718 & \textbf{15.35} & 205.53 & 170.86 & 16.50 & 156.63 \\
        \bottomrule
    \end{tabular}
    \end{center}
\end{table}

==> word_detector_table_vq01000.tex <==
\begin{table}[h]
\small
    \caption{Performance of the VQ3 layer from the ``$\{2\} \rightarrow \{2, 3\}$'' model when codes are treated as word detectors.}
    \label{tab:code_as_word_detect_init01000}
    \begin{center}
    \resizebox{.93\linewidth}{!}{
    \begin{tabular}{cccrrrrcrrrr}
        \toprule
        \multirow{2}{*}{rank} & 
        \multirow{2}{*}{code} & 
        \multicolumn{5}{c}{Top Hypotheses} & 
        \multicolumn{5}{c}{Second Hypotheses} \\
        & & word & F1 & P & R & occ & word & F1 & P & R & occ\\ 
        \cmidrule(lr){3-7} \cmidrule(lr){8-12}
        \midrule
  1 &  924 &     people &  76.71 &  67.49 &  88.85 &  1665 &   computer &   2.17 &   1.12 &  40.40 &    40 \\
  2 &  749 &      white &  76.47 &  66.92 &  89.21 &  2265 &        one &   4.15 &   2.50 &  12.14 &   134 \\
  3 &  530 &   building &  75.47 &  64.84 &  90.28 &  1681 &  buildings &  23.93 &  13.81 &  89.67 &   356 \\
  4 &  505 &       blue &  59.12 &  46.90 &  79.96 &  1093 &       pool &  10.74 &   5.89 &  60.80 &   152 \\
  5 &  581 &       snow &  57.61 &  41.77 &  92.83 &   466 &      snowy &  16.63 &   9.12 &  94.50 &   103 \\
 \multicolumn{12}{c}{$\cdots$}\\
198 &   38 &  structure &   5.62 &   6.20 &   5.14 &    13 &      graph &   4.03 &   2.19 &  25.00 &     2 \\
199 &  432 &    parking &   5.61 &   2.90 &  83.12 &   133 &       park &   5.56 &   2.87 &  82.89 &   126 \\
200 &  329 &   standing &   5.60 &   2.97 &  49.63 &   399 &      woman &   3.09 &   1.62 &  34.67 &   276 \\
        \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}
